Kharita: Robust Map Inference using Graph Spanners

The widespread availability of GPS information in everyday devices such as cars, smartphones and smart watches make it possible to collect large amount of geospatial trajectory information. A particularly important, yet technically challenging, application of this data is to identify the underlying road network and keep it updated under various changes. In this paper, we propose efficient algorithms that can generate accurate maps in both batch and online settings. Our algorithms utilize techniques from graph spanners so that they produce maps can effectively handle a wide variety of road and intersection shapes. We conduct a rigorous evaluation of our algorithms over two real-world datasets and under a wide variety of performance metrics. Our experiments show a significant improvement over prior work. In particular, we observe an increase in Biagioni f-score of up to 20% when compared to the state of the art while reducing the execution time by an order of magnitude. We also make our source code open source for reproducibility and enable other researchers to build on our work.

==> clustering.tex <==
\section{Clustering (1 page)}
\label{sec:clustering}
In this section we discuss the details on how we identify the clusters of close data points which represent segments of the road infrastructure. 


\subsection{Data}
Data we use to generate the map is crowdsourced by by a fleet of several hundred vehicles with attached GPS-enabled blackbox devices. These devices report a number of variables about the state of the car via a cellular network. The data is reported using timestamped records which are generated every 10 seconds (or less) including the following information:
the \textit{location} $(lon,lat)$ of the vehicle, the \textit{speed} and the \textit{heading} of the moving direction. Heading is measured in angles against the North axis in degrees reporting values from $0$  to $360^{\circ}$. Note that most of prior work on map inference \cite{} does not utilize the heading information even though it is standardly reported by GPS-enabled devices. 

The data used in this paper covers a rectangle (in $lat,lon$ coordinates) approximately 6km$\times$8km of urban region in the city of Doha with a mixture of highways, high and medium volume roads and capillary streets. Our data contains all the records generated by our fleet within this rectangle in October and November of 2015. We have overall around 12M datapoints, or 200K records per day. 

\textbf{RS: do we want to discuss privacy/annonimity issues of the data?}

\subsection{Preprocessing}
Our major preprocessing step is data densification. Namely, in low-volume road segments we may get very few data points which may turn the clustering process rather awkard. Hence, we artificially add datapoints along the trajectory of the moving vehicle in the following manner. If the two consequtive datapoints $X_1 = (lon_1,lat_1,\alpha_1)$, $X_2= (lon_2,lat_2,\alpha_2)$ on the trajectory have headings with angular difference of less than $5^{\circ}$ then we add $s$ datapoints points between them in an equidistant manner, where $s = \lfloor geodistance(X_1,X_2)/ 20m \rfloor$. By doing this we effectively create a point every (approximately) $20m$ along the pieces of the trajectories on the straight roads. 

We stress here that this densification step can be skipped if the data is dense enough, or the map accuracy in the low-frequency roads is not important for the end-user of the map. However, our design goal is to achieve high levels of map accuracy not only for arterial roads but also for minor streets too and we densify the original data before clustering. 

Overall our densification process roughly doubles the number of datapoints.

In addition to densification we identified a single vehicle in our dataset which produced abnormal location infromation (lat/lon shifted northeast by several hundred meters) and filtered it out of the dataset. 

\subsection{Clustering}
After the pre-processing stage, our input is transformed to the list of records in the form: $(user_-id, timestamp, lon, lat, heading)$. Our goal in this secion is to cluster together similar data points which fall in the same road segment. For clustering purposes we look at each data point independently; thus we do not use the trajectory information (inferred from the timestamps and $user_id$s) to cluster the points. These clusters will later be tied together using the trajectory information in the next section to form the road network. 

Our clustering is $k$-means with several modifications which we will detail below. The distance metric takes into account the location $L=(lat,lon)$ of the datapoint and the heading. For two points $(L_1,\alpha_1)$ and  $(L_2,\alpha_2)$ the distance is
\begin{equation}\label{eq:distancemetric}
d((L_1,\alpha_1),(L_2,\alpha_2)) = \sqrt{v(L_1,L_2)^2+ (\theta d_{\circ}(\alpha_1,\alpha_2))^2},
\end{equation}
where $v(L_1,L_2)$ is Vincenty distance in meters,  $d_{\circ}$ is the angle distance
\footnote{$d_{\circ}(\alpha_1,\alpha_2) = min(|\alpha_1-\alpha_2|,360^\circ-|\alpha_1-\alpha_2|)$.}
and $\theta$ is the heading penalty parameter. For most of the analysis in Sec \ref{} we set $\theta$ in such a way to penalize $180^\circ$ heading difference equivalently to $50m$ of geo distance. 

It is straighforward to check that the above distance measure satisfies the triangle inequality and is indeed a metric and its units are meters. \textbf{RS:Note to myself: we should evaluate different $\theta$ too!}

\textbf{Seed selection} The number of clusters is an unknown variable which we determine using the following process. We start with and empty seed list and go through the datapoints sequentially. For datapoint $(L,\alpha)$ if there is no seed which is withing $seed_-radius$ of $(L,\alpha)$ in our metric $d(\cdot)$, we add the datapoint to the seed list and continue iterating through the remaining datapoints. By doing so we spread seeds uniformly throughout space by making sure there are no two seeds within $seed_-radius$ of each other. \textbf{RS:Note to myself: we should evaluate different $seed_-radius$!}

\textbf{$k$-means clustering}. After the seeds are selected we run standard $k$-means algorithm (where $k$ denotes the number of seeds selected) where for the assignment step we use the metric $d$ defined by (\ref{eq:distancemetric}) and in the update step cluster centroid is updated using standard mean along the $lat/lon$ coordinates and the mean of circular quantities for the heading coordinate. Formally, for the cluster of points $S_{i}^{(t)}$ the centroid is:
$$m_{i}^{(t)} = (\overline{lat},\overline{lon},\overline{\alpha})$$ 
where:
$$\overline{lat} = \frac{1}{|S_{i}^{(t)}|}\sum_{(lat, lon, \alpha) \in S_{i}^{(t)}} lat.\ \ \ \  
 \overline{lon} = \frac{1}{|S_{i}^{(t)}|}\sum_{(lat, lon, \alpha) \in S_{i}^{(t)}} lon $$
and 
$$\overline{\alpha} = atan2(\frac{1}{|S_{i}^{(t)}|}\sum_{(lat, lon, \alpha) \in S_{i}^{(t)}} \sin\alpha ,\frac{1}{|S_{i}^{(t)}|}\sum_{(lat, lon, \alpha) \in S_{i}^{(t)}} \cos\alpha).$$
\textbf{RS:As I was writing i realized that mean od circular quantities may or may not (more likely not) be the least-square estimator for the angle distance metric $d_{\circ}$. Something to check!}. We iterate $k$-means until the cost reduction becomes smaller than 0.0001 times cost. The final result of the $k$-means is a set of $k$ clusters which represent different road segments. Some clusters represent straight road segments and among them the variability of the heading angles among the points within the cluster is indeed very small (around $1-2^\circ$). However, clusters around intersections and roundabouts contain points with a wider range of angles which may confuse the road creation process (Section \ref{}). Hence we have the final step in the clustering phase:

\textbf{Large heading variability cluster split.} To narrow down the clusters which have large heading angle variability we simply split them. For a cluster $i$ with mean heading $\alpha_i$ we define heading variability $hv_i$ as the average of $d_{\circ}(\alpha,\alpha_i)$, across all points within the cluster\footnote{Note that angular arithmetics does not allow us to use ore standard measures of variability like standard variation or variance.}. If the heading variability of cluster $i$, $hv_i$ is greater than $10^\circ$ we split it in two using 2-means clustering of the angles and calculate the centroids of the new clusters accordingly. 





\subsection{Postprocessing}
Update centroids through splines or other methods before passing it to graph construction


==> incrementalUpdate.tex <==
\section{Incremental Map Maintenance (1 page)}
\label{sec:incrementalMapMaintenance}

\subsection{Approach 1: Incremental KMeans based}

\subsection{Approach 2: Trajectory based}


==> metadataInference.tex <==
\section{Metadata Inference (0.5 page)}
\label{sec:metadataInference}

